Behavioral Use Licensing for Responsible AI

With the growing reliance on artificial intelligence (AI) for many different applications, the sharing of code, data, and models is important to ensure the replicability and democratization of scientific knowledge. Many high-profile academic publishing venues expect code and models to be submitted and released with papers. Furthermore, developers often want to release these assets to encourage development of technology that leverages their frameworks and services. A number of organizations have expressed concerns about the inappropriate or irresponsible use of AI and have proposed ethical guidelines around the application of such systems. While such guidelines can help set norms and shape policy, they are not easily enforceable. In this paper, we advocate the use of licensing to enable legally enforceable behavioral use conditions on software and code and provide several case studies that demonstrate the feasibility of behavioral use licensing. We envision how licensing may be implemented in accordance with existing responsible AI guidelines.

==> samples/notes.tex <==
% \section{Openness is Good, When Done Thoughtfully} [DANIEL,JULIA,BRENT, DANISH]

% \begin{itemize}
% \item AI has seen rapid advances thanks to the availability of data, scalable computation/hardware and new algorithms. 

% \item Sharing code is good - it helps science, improve confidence in research, etc.

% \item Examples: NeurIPS expects code with submissions and accepted papers.

% \item However, code is becoming more and more powerful AND multipurpose.
% Give examples of some of the papers that were accepted to late NeurIPS.

% \item People need to think through the consequences of releasing code.
% They could really do with a framework and practical tools to help them.

% \item It is not enough to say ``not for commercial use" or ``MIT License" etc.

% \item What do current licenses do?  They control how the code is distributed and how things made from the code are distributed.  NOT other behaviors of the people using the code.
% \end{itemize}
%The computer science, and more specifically for our purposes Machine Learning and AI communities, are no exception. 
%Sharing code and data allows researchers and developers to collaborate on solutions for bigger problems

%\dan{I think the arguments that code/data sharing allow research to be vetted, better understood and built upon is a better one here than the arguement below.}
%Sharing code and data allows researchers and developers can collaborate to solve big, global problems and make progress towards the common good. But there is growing concern around how to enable this while also preventing misuse or inappropriate use. %In addition,  as well as deal with the issues with bias, inadequate testing and generalization % in areas such as surveillance, media, and security. 
%\dan{}

%\dan{Suggested high-level structure in the introduction: 1) Sharing is necessary for science and should be encouraged - increases transparency, replicability, efficiency, and shared knowledge. - In some cases e.g., GPT-3 sharing is the only way, impossible for many people to reproduce. 2) However, sharing creates opportunities for misuse.  3) Currently, there are no good ways of controlling behavior. 4) We argue for enforceable behavioral use licenses and furthermore for a set of easy to use licenses.  Do you think we need to make this specific to neural models? It is probably assumed in the current work but will eventually be superseded.}

==> unused/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> unused/README.tex <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts
		


==> unused/commented_text.tex <==
For camera ready, I am moving commented things here:



recall-heavy, low-precision facial recognition technologies may be acceptable under some circumstances for use in finding missing persons from CCTV footage\footnote{https://in.reuters.com/article/us-india-crime-children/indian-police-use-facial-recognition-app-to-reunite-families-with-lost-children-idUSKBN2081CU}, but may be inappropriate for associating an individual to the scene of a crime\footnote{https://www.theverge.com/2020/6/24/21301759/facial-recognition-detroit-police-wrongful-arrest-robert-williams-artificial-intelligence}.


Regardless of the opinions about whether these models memorize or ``learn'' language\footnote{https://www.technologyreview.com/2020/08/22/1007539/gpt3-openai-language-generator-artificial-intelligence-ai-opinion/}, it is undeniable that they produce impressive language output.
%As a result, this model will be used for many downstream tasks, not only because it shows good performance, but also because very few organizations will be able to train a model of similar size.  



%\noindent{\bf Contributions:} In this paper we motivate the use of licensing as a mechanism for enabling {\em legally enforceable}[?] responsible-use. We present exemplar clauses based on recent ethical guidelines such as the Montreal Declaration for Responsible-AI\cite{} as well as based on use-cases that have been widely accepted as harmful or have unintended consequences. In addition, we also include a case-study(?) to demonstrate how licensing clauses could be informed based on the data included in an AI factsheet of an AI system.


%For the discussion in this paper we categorise existing work on ``responsibility'' in AI based on how they apply to three crucial development activities: %evelopment decisions that need to be made when dei %towards making AI system decision interpretable and explainable.  resulting in a wide mix of tools and frameworks that have their own interpretation of `responsible'.  has been difficult for the AI community to universally define what it means for AI to be `responsible'. Unlike regular software systems where models can be debugged, thoroughly tested, have software defects fixed and verified, AI systems do not offer the same degree of control and neither are there run-time guarantees of system behaviour at deployment. The deployment characteristics of an AI system is affected by three sets of decisions made during its development:
% \begin{itemize}
%     \item {\bf Data used for training:} An AI system is affected by the data it has been trained on. Eg: A classifier trained on black and white images will not work well on colour images. 
%     \item {\bf Model design and architecture:} Models may be designed to be {\em explainable} or {\em interpretable}, or may be a black-box model. % without interpretable decision making/result generation. 
%     Eg: A Question-Answering system which returns the evidence for an answer from a text document, as opposed to one that only returns a keyword answer. 
%     \item {\bf Evaluation of limitations and risks:} Apart from optimizing the parameters of a model based on a mathematical objective, AI systems may be qualitatively assessed for performance on an end-task. This can often present insights into possible failure-points arising due to data bias or model design. Eg: If a classifier trained to distinguish between a wolf and a dog where the training data consisted of images of wolves in the wild, and dogs indoors. A model may incorrectly assume that the background is indicative of the animal class.
% \end{itemize}


% \begin{figure*}
% %  Requires \usepackage{graphicx}
% \center
%   \includegraphics[scale=0.5]{samples/figs/ResponsibleAI_Ecosystem.jpg}
%   \caption{The responsible AI ecosystem contains growing number of tools, including: ethical standards, approaches from mitigating bias and increasing interpretibility and explainablity, data and fact sheets for detaining algorithms and training data. We advocate for the use of licensing as a mechanism for enabling AI developers to incorporate permissive and restrictive-use clauses to help promote responsible use. }%Responsible AI Ecosystem}\label{fig:ecosystem}
% \end{figure*}
%The AI community has developed tools and frameworks that are aimed one or more of these developmental We find that the AI community has attempted to define `responsible' by addressing issues that arise from one or more of these decision steps. We classify the approaches into three categories: (i) Toolkits and Best Practices for AI development (ii) Algorithm Development for interpretiblity, explainability and trust (iii) Mechanisms for Promoting appropriate-use. 


%Thus, the question remains: Should technology creators in the AI space be especially mindful of what they are enabling with their technology? Should such technology creators engage in more proactive attempts of downstream regulation using mechanisms like license clauses in order to encourage or impose more responsible behaviors?  If the answers are ``yes,'' what license terms should we encourage and normalize to allow for behavioral use restrictions to be placed on AI code, models or data? 
